The Multiscale Laplacian Graph Kernel

Many real world graphs, such as the graphs of molecules, exhibit structure at multiple different scales, but most existing kernels between graphs are either purely local or purely global in character. In contrast, by building a hierarchy of nested subgraphs, the Multiscale Laplacian Graph kernels (MLG kernels) that we define in this paper can account for structure at a range of different scales. At the heart of the MLG construction is another new graph kernel, called the Feature Space Laplacian Graph kernel (FLG kernel), which has the property that it can lift a base kernel defined on the vertices of two graphs to a kernel between the graphs. The MLG kernel applies such FLG kernels to subgraphs recursively. To make the MLG kernel computationally feasible, we also introduce a randomized projection procedure, similar to the Nystr\"om method, but for RKHS operators.

==> alg2.tex <==
\begin{algorithm*}[]
\begin{algorithmic}
\STATE \textbf{INPUT:} A collection of graphs \m{\Gfrak=\cbrN{\sseq{\Gcal}{M}}} with 
joint vertex set \m{\wbar V}, a base kernel \m{\kappa\colon \wbar V\times \wbar V\to\RR}, 
\STATE~~~ a system of nested subgraphs \m{ v\tin N_1( v)\subseteq N_2( v)\subseteq \ldots \subseteq N_L( v)} for each vertex \m{ v\tin \wbar V}, and
\STATE~~~ smoothing parameters \m{\eta} and \m{\gamma}.
\STATE 
\STATE \textbf{Sample}~ \m{\cbrN{\sseq{\tilde v}{\tilde N}}}\: from \m{\wbar V} 
\STATE \textbf{Compute}~ the subsampled Gram matrix \m{\tilde K}, with elements \m{\tilde K_{i,j}\<=\kappa(\tilde v_i,\tilde v_j)} 
\STATE \textbf{Compute}~ a basis \m{\cbr{\sseq{\xi}{\tilde P}}} for the approximate joint feature space \m{\tilde W} from \m{K} 
%\STATE \textbf{Compute}~ \m{\tilde W_\kappa},\; the subsampled \m{\tilde P} dimensional 
%approximate joint feature space (Definition \ref{def: randomized})
\STATE \textbf{For each (} \m{ v\tin \wbar V} \textbf{) \{}~ \m{\V \phi( v)\leftarrow }~  
the projection of \m{\phi_\kappa( v)} to \m{\tilde W_\kappa} \textbf{\}}
\STATE 
\STATE \textbf{For (} \m{\ell\<=1} \textbf{to} \m{L} \textbf{) \{}
\STATE~~~ \textbf{For each (} \m{ v\tin \wbar V} \textbf{) \{}
\STATE~~~~~~ \m{\Lcal_{ v}\leftarrow} the Laplacian of \m{G_\ell( v)}~ %\textbf{\}}
%\STATE~~~ \textbf{For each (} \m{v\in \wbar V} \textbf{) \{}~ \m{
\STATE~~~~~~ \m{U_{ v}\leftarrow [\V\phi(w_1),\ldots,\V\phi(w_{\abs{\!G_\ell( v)\!}})]^\top},\;
where \m{(\sseq{w}{\abs{\!G_\ell( v)\!}})} are the vertices of \m{G_\ell( v)}~ %\textbf{\}}
%\STATE~~~ \textbf{For each (} \m{v\in \wbar V} \textbf{) \{}~ 
\STATE~~~~~~ \m{\wbar S_{ v}\leftarrow U_v(\Lcal_{ v}+\eta I)^{-1} U_v^\top+\gamma I}~ %\textbf{\}}
\STATE~~~ \textbf{\}}
\STATE~~~ \textbf{Sample}~ \m{\cbrN{\sseq{\tilde v}{\tilde N}}}\: from \m{ V} 
\STATE~~~ \textbf{Compute}~ the subsampled Gram matrix \m{\tilde K\tin\RR^{\tilde N\times \tilde N}}, with elements 
\[\tilde K_{i,j}=\kflg(G_\ell(\tilde v_i),G(\tilde v_j))=
\fr{\absbig{\nts \brbig{\ovr{2}\wbar{S}_{\tilde v_1}^{-1}\<+\ovr{2} \wbar{S}_{\tilde v_2}^{-1}}^{-1}\nts }^{1/2}}
{\absN{\nts \wbar{S}_{\tilde v_1}\nts }^{1/4}\; \absN{\nts \wbar{S}_{\tilde v_2}\nts }^{1/4}}
\]
\STATE~~~ \textbf{Compute}~ a basis \m{\cbr{\sseq{\xi}{\tilde P}}} for the approximate joint feature space \m{\tilde W_\kappa} from \m{K}
\STATE~~~ \textbf{For each (} \m{ v\tin \wbar V} \textbf{) \{}~ \m{\V \phi( v)\leftarrow }~  
the projection of \m{\phi_\kappa( v)} to \m{\tilde W_\kappa} \textbf{\}}
\STATE\textbf{\}}
\STATE

\STATE \textbf{For (} \m{i\<=1} \textbf{to} \m{M} \textbf{) \{}
\STATE~~~ \m{\Lcal_{i}\leftarrow} the Laplacian of \m{\Gcal_i}
\STATE~~~ \m{U_{i}\leftarrow [\V\phi(v_1),\ldots,\V\phi(v_{\abs{\!V_i\!}})]^\top},\;
where \m{(\sseq{v}{\abs{\!V_i\!}})} are the vertices of \m{\Gcal_i}
\STATE~~~ \m{\wbar S_{i}\leftarrow U_i(\Lcal_{ i}+\eta I)^{-1} U_i^\top+\gamma I}
\STATE\textbf{\}}
\STATE 
\STATE\textbf{Compute}~ the MLG Gram matrix \m{G\tin\RR^{M\times M}}, with elements 
\[G_{i,j}=\kmlg(\Gcal_i,\Gcal_j)=
\fr{\absbig{\nts \brbig{\ovr{2}\wbar{S}_{i}^{-1}\<+\ovr{2} \wbar{S}_{j}^{-1}}^{-1}\nts }^{1/2}}
{\absN{\nts \wbar{S}_{i}\nts }^{1/4}\; \absN{\nts \wbar{S}_{j}\nts }^{1/4}}
\]

\STATE \textbf{OUTPUT:} the MLG Gram matrix \m{G}
\end{algorithmic}
\caption{\label{alg1}~The fast MLG algorithm (high level overview)}
\end{algorithm*}

